FedFNN: Faster Training Convergence Through Update Predictions in Federated Recommender Systems

Federated Learning (FL) has emerged as a key approach for distributed machine learning, enhancing online personalization while ensuring user data privacy. Instead of sending private data to a central server as in traditional approaches, FL decentralizes computations: devices train locally and share updates with a global server. A primary challenge in this setting is achieving fast and accurate model training - vital for recommendation systems where delays can compromise user engagement. This paper introduces FedFNN, an algorithm that accelerates decentralized model training. In FL, only a subset of users are involved in each training epoch. FedFNN employs supervised learning to predict weight updates from unsampled users, using updates from the sampled set. Our evaluations, using real and synthetic data, show: 1. FedFNN achieves training speeds 5x faster than leading methods, maintaining or improving accuracy; 2. the algorithm's performance is consistent regardless of client cluster variations; 3. FedFNN outperforms other methods in scenarios with limited client availability, converging more quickly.

==> source/disc-concl.tex <==
\section{Discussions and Conclusions}
\label{sec:disc}
This paper presents \texttt{FedFNN}, a new framework in Federated Learning, which speeds up the training of machine learning models, with a focus on the recommender systems.
Although we emphasise its applications on recommender systems, the same methodology could be applied to other areas.
Our \texttt{FedFNN} framework predicts the weight updates for clients not available during training, increasing the performance of the model, especially at the early stage of the process.
Comparing with the current state-of-the-art, \texttt{FedFNN} proves to be not only faster, but provides higher accuracy with the same amount of training rounds.
Moreover, \texttt{FedFNN} is shown to perform optimally in conditions where the sample size is relatively small or when some clients present poor availability.
We also demonstrate empirically that training \texttt{FedFNN} over input data presenting a high number of clustered preferences (e.g. distinct group of clients with distinguishable preferences) is still beneficial when compared with existing alternatives. Given its novelty, there are several limitations of our model that can be address in the future work.
Firstly, it is trained with offline data (ratings or preferences existing before the start of the training), which does not include any online interactions. 
%
%For future work, we plan to extend this setting to include a more realistic scenario of online ratings during training. We introduce \texttt{FedFNN} in the context of recommendation algorithms based on matrix factorization, which is a popular approach but not the most accurate in the current literature. In the future, we will consider the adaptation of other approaches, which represent the state-of-the-art for the recommendations tasks, like graph neural networks approaches (GNN) or Deep \& Cross Networks  (DCN) \cite{wu2021fedgnn, wang2021dcn}.
%
For future work, we plan to extend this setting to include online ratings during training. 
We introduce \texttt{FedFNN} in the context of recommendation algorithms based on matrix factorisation.
Although matrix factorisation remains a popular approach in the literature, a new family of algorithms based on deep neural networks recently gaining traction. 
In the future, we will consider the adaptation of \texttt{FedFNN} to these approaches, such as graph neural networks (GNN) or Deep \& Cross Networks  (DCN) \cite{wu2021fedgnn, wang2021dcn}. \texttt{FedFNN} has a significant impact on the first iterations of the model.
However, it lacks of personalisation when predicting the updates because it optimises the root mean square error of the weights updated predictions during its training.
%
We hope to see future work that is able to consider personalization while still improving its accuracy and speed of convergence.
%
Also, in our setting we assume a static learning rate and discount factor; this choice may not be optimal 
since the amount of information should be adapted along the training. 
Adaptive learning rates and further investigation into the discount factor are needed to improve the robustness of the model.



==> source/experiments.tex <==
\section{Experiments}
\label{sec:exp}

\begin{figure*}[t]

    \centering
    \includegraphics[width=.75\linewidth]{plots/comparison/comparison-legend.pdf}\\

    \begin{tabular}{cccc}
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/ml-100k_100-HR10.pdf} &
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/ml-100k_100-nDCG10.pdf}&
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/ml-100k_500-HR10.pdf} &
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/ml-100k_500-nDCG10.pdf}\\
    \end{tabular}
    (i) ML-100k 
    \begin{tabular}{cccc}
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/yelp_100-HR10.pdf} &
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/yelp_100-nDCG10.pdf}&
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/yelp_500-HR10.pdf} &
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/yelp_500-nDCG10.pdf}\\
    \end{tabular}
    (ii) YELP
    \begin{tabular}{cccc}
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/amazon_100-HR10.pdf} &
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/amazon_100-nDCG10.pdf}&
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/amazon_500-HR10.pdf} &
    \hspace{-3mm}\includegraphics[width=0.25\linewidth]{plots/comparison/amazon_500-nDCG10.pdf}\\
    \end{tabular}
    (ii) AMAZON

\caption{Comparison of FL models on three different datasets. The first two columns show only the first 100 iterations, while the third and fourth columns are showing up to 500 iterations.}
    \label{fig:comparison}
    \vspace{-3mm}
\end{figure*}

This section focuses on answering the following research questions: $(RQ1)$ What is the performance of \texttt{FedFNN} compared to the state-of-the-art in terms of accuracy and speed of convergence?; $(RQ2)$ Do the different strategies for updating both user and item embeddings significantly  increase the speed of convergence for FL models?; $(RQ3)$ How might distribution of user preferences affect the performances of \texttt{FedFNN}?; $(RQ4)$ How might client availability and sample size impact the performances of \texttt{FedFNN}?

\noindent \textbf{Data.} For the experimental section we use 3 different datasets: MovieLens, a popular movies reviews' collection used for bench-marking recommendation algorithms (\textbf{ML-100K}); Yelp, an aggregator of shops reviews (\textbf{YELP}); Amazon Music sample of songs reviews (\textbf{AMAZON}). The characteristics of the 3 datasets are summarised in Table \ref{tab:summary}.

\begin{table}[h]
% \resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
 \textbf{Dataset} & \textbf{Interactions} &  \textbf{Users} &  \textbf{Items} &  \textbf{Sparsity} \\
\midrule
AMAZON &        64,706 &   5,541 &   3,568 &    0.0135 \\
ML-100K &       100,000 &    943 &   1,682 &    0.0630 \\
YELP &       267,211 &  16,442 &  11,128 &    0.0015 \\
\bottomrule
\end{tabular}
% }
\caption{Summary of data used for the experiments}
\label{tab:summary}
\end{table}

\noindent \textbf{Algorithms.} We test \texttt{FedFNN} with state-of-the-art algorithms and a baseline: 

\begin{itemize}

\item\texttt{FedFast}: the current state-of-the-art, in terms of speed, to the best of our knowledge. It predicts the subordinates through a clustering based approach (\cite{fedfast});

\item\texttt{FedAvg}: baseline on which \texttt{FedFNN} and \texttt{FedFast} have been designed. It distributes local updates (both item and client embeddings) through averaging, and does not predict embeddings of the subordinate clients (\cite{mcmahan2017communication});

\item\texttt{WCU}: \emph{Without Client Updates} (WCU) algorithm only updates the embeddings of the sampled clients and the items that have been interacted with; subordinate embeddings are not updated. We include this option to emphasise the differences in performances with \texttt{FedFast}, which the only difference is the inclusion of the clustering method for predicting the unsampled clients.

\item\texttt{GMF}: the centralised version of the Neural Matrix Factorisation algorithm. It is included to establish the upper-bound of the FL-based solutions \cite{he2017neural}.

\item\texttt{FedFNN-MLP}: \texttt{FedFNN} implementation using a multi-layer perceptron (MLP) to predict the unsampled clients.

\item\texttt{FedFNN-MLP-CV}: the architecture is the same of FedFNN-MLP, but this time the hyperparameters of \texttt{FedFNN} (dropout, number of hidden neurons, number of layers) are optimised running a grid-search in a 5-fold cross validation, at each training round.

%\item\textbf{FedFNN-MLP-3T}: in this case, the architecture is the same of standard FedFNN, but using as input data the last three updates of the sampled clients.


\end{itemize}

For the item embedding updates it is important that an optimal strategy for redistributing the new item updates $(v^{t+1}[k])$ through a weighted average is found. For this reason we test different item embedding updates (\textbf{W0, W1} and \textbf{W2}).

\subsection{Performance and Accuracy (RQ1, RQ3)} 

\paragraph{Accuracy and Convergence Comparison.}

Here we compare different \texttt{FedFNN} implementations with the algorithms and datasets introduced above. In Figure \ref{fig:comparison} we show the results generated after both 100 and 500 iterations, where the first two columns of plots show the first 100 iterations (HR@10 and nDCG@10), while the second and third columns show the whole training rounds. 
%
In order to generate a fair comparison: $(i)$ for each dataset, the learning rate of the local updates is the same for all the algorithms; $(ii)$ W1 is the item embedding strategy used for \texttt{FedFast}, \texttt{FedFNN} and \texttt{WCU} implementations; $(iii)$ the sample size of the local updates is fixed to $10\%$ for all the experiments.

Overall, \texttt{FedFNN-MLP} consistently outperforms the other algorithms on all 3 datasets, both in terms of speed of convergence (the number of iterations needed to reach stable level of convergence), and final accuracy (the final NDCG and HR). In our experiments we focus on the first 100 iterations of training to check the speed of convergence during this early stage: with ML-100K data, \texttt{FedFNN-MLP} is 2x faster than \texttt{FedFast}, for YELP data it is 5x faster, and for AMAZON it is even 8x faster than \texttt{FedFast}. Specifically, \texttt{FedFNN-MLP} needs only 12 iterations to reach \texttt{FedFast} accuracy at the 100th iteration. 
%
On the other hand, \texttt{FedFast} is better than \texttt{FedAvg} in terms of performance and accuracy, but presents similar performances of \texttt{WCU}, which is characterised by the absence of clustering techniques. This means that the clustering approach used to predict the clients' embeddings appears to have little effect on the performance of the algorithm.

The introduction of the cross validation for \texttt{FedFNN}, helps to generate robust predictions (\texttt{FedFNN-MLP-CV}), presenting an increase in performance in the early stage of training, for all the experiments. In the case of MovieLens dataset, \texttt{FedFNN-MLP-CV} is also slightly improving the overall performance of the standard \texttt{FedFNN-MLP}.

\smallskip
\mybox{mygray}{ \begin{observation} \texttt{FedFNN} outperforms \texttt{FedFast} both in terms of accuracy and speed of convergence. \texttt{FedFast} and \texttt{WCU} result in comparable performance,which demonstrates the negligible improvement gained by adopting a clustering scheme for embedding predictions. Cross validation helps to speed up \texttt{FedFNN} algorithm in the early stage of the training.
 \end{observation}
 }
\smallskip

\paragraph{Grouped Preferences.} In order to analyse the performance of \texttt{FedFNN} in presence of clustered preferences we design a synthetic data generator which allows to input the number of groups of users presenting same preferences when generating the user-item interactions. 
%
We can first indicate the desired number of users (N) and items (M), then a mapping function $\ell : D \rightarrow \{D_1, D_2, ... D_G\}$, which maps each user-item interaction to a different subset $D_j$, where G is the total number of groups in input. 
%
For sake of simplicity, group of users do not overlap in terms of item preferences an all the groups have the same relative size. 
%
To generate more realistic data, we include parameters to model sparsity and popularity as a power-law distribution, which is generated through a \emph{Beta(a,b)} random variable. 
%
First, we use the Beta (with parameters fixed to $a = 1, b=3$) for generating the deviation from the average $s$ for all users, then, we assign to each user $u$ the final level of sparsity $s_u = s + s(s_u - s_M)$, where $s_M$ is the median of the sparsity vector generated through the sampling. 
%
The \emph{Beta} parameters are chosen to lead to a level of sparsity similar to the one in the real dataset introduced in Table 1.
%
For each group of items $D_j$, we can define a different popularity bias vector, $\mathbf{p}_j$ which for each item $i$ in the group $j$, maps a coefficient $p_j(i) \in [0,1]$ representing the chances of being selected. In this way, when generating user preferences, first the number of interactions is computed ($n_u = \ceil{M\times s_u}$) and then $n_u$ items are sampled following $\mathbf{p}_j$.
The detailed process follows:
\begin{enumerate}
\item We initialise the number of users $N$, the number of items $M$, the sparsity value $s$ and the number of groups G. Initialise the sparsity sample and generate the sparsitiy value for each user ($s_u$).

\item for each group we generate the popularity vector $\mathbf{p}_j$, sampling from the beta distribution.

\item for each user we then sample $n_u$ items following the probability:
$$
p(u,i) = \frac{h(u,i) p_i }{\sum_{j \in I} h(u,j) p_j}
$$
where $h(u,i) = \eta$ if $u$ and $i$ are mapped through $\ell(.)$ to the same group, otherwise $h(u,i) = (1- \eta)$. This parameter introduces a certain level of randomness, to have more realistic clusters distribution. In our experiments, we fix it to $\eta = 0.9$.  
\end{enumerate}


We test \texttt{FedFNN} and \texttt{FedFast} on 6 different datasets, which differ only by the number of input clusters, where $G\in \{ 5, 10, 50, 100, 500,  1000\}$. In this case, \texttt{FedFast} is trained given in input the exact number of clusters used to generate the data. Also the parameters used to generate sparsity and popularity bias are the same along all the datasets. The sample size and local learning rate for the training of the algorithm does not change for the experiments. The results are presented in the Figure\ref{fig:clusters}, where the metric used is the difference in performance between \texttt{FedFNN} and \texttt{FedFast}, i.e. $\Delta_{HR}$ and $\Delta_{nDCG}$, positive if \texttt{FedFNN} presents better accuracy, negative if \texttt{FedFast} is more accurate. This value is measured at three different moments along the training: at early stage (after 100 iters); in the middle (after 300 iterations) and at the end of the training (after 500 iterations). It is possible to highlight how \texttt{FedFNN} is consistently better in terms of accuracy, looking at the values of $\Delta_{HR}$ and $\Delta_{nDCG}$. The improvement of \texttt{FedFNN} over \texttt{FedFast} is most noticeable in the early stages of learning (at 100 iterations), but even at later stages (after 300 and 500 iterations) it is consistently better in terms of accuracy. Since through the local updates, the two algorithms can only access to a portion of the whole dataset, the clustering approach (\texttt{FedFast}) may struggle to sample necessary information to properly assign the clients to the right clusters.

\smallskip

\mybox{mygray}{ \begin{observation} In the presence of both a low and high number of clustered preferences, \texttt{FedFNN} is consistently faster and also more accurate than \texttt{FedFast}.
 \end{observation}
 }

\smallskip

\begin{figure}[h]
    \centering
    \begin{tabular}{cc}
        \hspace{-3mm}\includegraphics[width=.45\linewidth]{plots/synth/HR-synth.pdf}
        \hspace{-3mm}\includegraphics[width=.45\linewidth]{plots/synth/nDCG-synth.pdf} 
    \end{tabular}

\caption{Comparsion of FedFast and \texttt{FedFNN} performances when users present different grouped preferences.}
    \label{fig:clusters}
\end{figure}


\subsection{Ablation Study (RQ2)}
In order to study the contribution of the algorithm proposed, we perform an ablation study to emphasise the importance of using different strategies for both client and item embedding updates. For this reason we test three different strategies of subordinates predictions (\texttt{FedFNN}, \texttt{FedFast} and \texttt{WCU}) and three different strategies of item embedding updates (W0, W1 and W2). The experiments are performed following the same configurations used in Figure \ref{fig:comparison}. In Table \ref{table:ablation} we present the results for MovieLens and Yelp datasets, highlighting accuracy (HR@10 and nDCG @10) after 100, 300 and 500 iterations. About item embedding updates, for both datasets, \textbf{W1} presents better performances, in terms of speed and accuracy. Moreover, W2 presents better performances when compared to W0, which is consistently the slower one, no matter the choice of client predictions strategy. Among the client updates, \texttt{FedFNN} is optimal in terms of accuracy and speed of convergence, for both datasets, at all stages of training. \texttt{FedFast} and \texttt{WCU} demonstrate similar performance. 

\smallskip
\mybox{mygray}{ \begin{observation} The client updates performed through \texttt{FedFNN} are consistently more accurate than those performed by \texttt{FedFast} and \texttt{WCU} in all the training phases (early, middle and late phases). In addition, the predictions made via the clustering approach (\texttt{FedFast}) do not differ from the ones generated with the baseline (\texttt{WCU}). Also, item embeddings benefit from a strategy exploiting clients presenting larger updates (\textbf{W1}), rather than either simple averaging through updates (\textbf{W0}) or considering user interactions (\textbf{W2}). 
 \end{observation}
 }
\smallskip

\begin{table}[h]
%\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
\multicolumn{7}{c}{ML-100k}\\
\midrule
\multirow{2}{*}{Model} &  \multicolumn{2}{c|}{100 iter} &  \multicolumn{2}{c|}{300 iter} & \multicolumn{2}{c}{500 iter} \\
{} &  HR@10  &  nDCG@10  &  HR@10  &  nDCG@10 & HR@10  &  nDCG@10 \\
\midrule

W0+WCU     &  0.4740 &    0.2636 &  0.6352 &    0.3859 &  0.7137 &    0.4331 \\
W0+FedFast &  0.4995 &    0.2826 &  0.6691 &    0.4060 &  0.7158 &    0.4299 \\
W0+FedFNN &  \textbf{0.5801} &    \textbf{0.3421} &  \textbf{0.6893} &    \textbf{0.4180} &  0.7063 &    \textbf{0.4365} \\

\midrule

W1+WCU      &  0.5981 &    0.3487 &  0.7444 &    0.4445 &  0.7678 &    0.4666 \\
W1+FedFast  &  0.5790 &    0.3255 &  0.7264 &    0.4435 &  0.7614 &    0.4620 \\
W1+FedFNN  &  \textbf{0.7084} &    \textbf{0.4281} &  \textbf{0.7667} &    \textbf{0.4755} &  \textbf{0.7890} &    \textbf{0.4942} \\

\midrule
W2+WCU      &  0.5451 &    0.3050 &  0.7137 &    0.4262 &  0.7561 &    0.4648 \\
W2+FedFast  &  0.5323 &    0.2904 &  0.7010 &    0.4148 &  0.7529 &    0.4551 \\
W2+FedFNN  &  \textbf{0.6225} &    \textbf{0.3616} &  \textbf{0.7222} &    \textbf{0.4425} &  \textbf{0.7614} &    \textbf{0.4768} \\
\midrule
\multicolumn{7}{c}{Yelp}\\
\midrule
W0+WCU     &  0.1999 &    0.0916 &  0.2013 &    0.0921 &  0.2048 &    0.0952 \\
W0+FedFast &  0.2030 &    0.0937 &  0.2101 &    0.0977 &  0.2163 &    0.1021 \\
W0+FedFNN  &  \textbf{0.2147} &    \textbf{0.0986} &  0.2094 &    0.0975 &  \textbf{0.2241} &    \textbf{0.1058} \\
\midrule
W1+WCU      &  0.5042 &    0.2918 &  0.5768 &    0.3404 &  0.5880 &    0.3513 \\
W1+FedFast  &  0.5017 &    0.2895 &  0.5774 &    0.3403 &  0.5876 &    0.3491 \\
W1+FedFNN  &  \textbf{0.5910} &    \textbf{0.3488} &  \textbf{0.6123} &    \textbf{0.3703} &  \textbf{0.6342} &    \textbf{0.3902} \\

\midrule
W2+WCU      &  0.2036 &    0.0927 &  0.2890 &    0.1506 &  0.3963 &    0.2319 \\
W2+FedFast  &  0.2053 &    0.0937 &  0.2729 &    0.1373 &  0.3895 &    0.2262 \\
W2+FedFNN   &  \textbf{0.3099} &    \textbf{0.1636} &  \textbf{0.4082} &  \textbf{0.2381} &  \textbf{0.4385} &  \textbf{0.2606} \\

\bottomrule
\end{tabular}
%}
\caption{Summary of the ablation study conducted to analyse the impact of user and item embedding updates.}
    \label{table:ablation}
\end{table}


%\begin{figure}[h]
%
%    \centering
%    \includegraphics[width=.6\linewidth]{plots/ablation/ablation-legend.pdf}\\
%
%    \begin{tabular}{ccc}
%    AVG & W1 & W2\\
%    \hspace{-3mm}\includegraphics[width=0.3\linewidth]{plots/ablation/ml-100k_avg_nDCG10.pdf} &
%    \hspace{-3mm}\includegraphics[width=0.3\linewidth]{plots/ablation/ml-100k_weighted1_nDCG10.pdf} & 
%    \hspace{-3mm}\includegraphics[width=0.3\linewidth]{plots/ablation/ml-100k_weighted2_nDCG10.pdf}
%    \end{tabular}\\
%    (i) ML-100k 
%    \begin{tabular}{ccc}
% 
%    \hspace{-3mm}\includegraphics[width=0.3\linewidth]{plots/ablation/yelp_avg_nDCG10.pdf} &
%    \hspace{-3mm}\includegraphics[width=0.3\linewidth]{plots/ablation/yelp_weighted1_nDCG10.pdf} & 
%    \hspace{-3mm}\includegraphics[width=0.3\linewidth]{plots/ablation/yelp_weighted2_nDCG10.pdf}\\
%
%    \end{tabular}	\\
%    (ii) YELP
%
%
%\caption{Ablation study which compares 3 strategies of item-embedding updates and 3 subordinate users predictions.}
%    \label{fig:ablation}
%    \vspace{-3mm}
%\end{figure}


\subsection{Poor availability and Sampling (RQ4)}

 We explore two different scenarios which are of practical significance in a FL setting: $(i)$ limited availability of clients, where along the training a group of client is consistently less available to be sampled (e.g. clients penalised when sampling the subset for the local updates); $(ii)$ a smaller fraction of clients are sampled to participate in training.

\paragraph{Availability.} Not all clients will have the same levels of availability during training, and those who participate less in training will have a diminished performing model. It is for this reason we decided to test how clients who participate less respond to the \texttt{FedAvg}, \texttt{FedFast} and \texttt{FedFNN} algorithms. Using ML-100K dataset, we split (uniformly at random) the clients in two blocks of same size. One block is fully available along the training (\textbf{normal availability}), while all the clients belonging to the other have 25\% chance of being available at each iteration for being sampled and run the local update (\textbf{poor availability}). Partitioning the clients this way means that the clients assigned to the poor availability group are consistently sampled and locally updated less frequently than the other group. We test and monitor the performances of three different models in this case (\texttt{FedFNN}, \texttt{FedFast} and \texttt{FedAvg}). In Figure \ref{fig:pooravail} we report on the left (Fig. 4a) the performance for the portion of users consistently available, while on the right (Fig. 4b) the performance of the sample \emph{poorly available}. \texttt{FedFNN} shows better performances for the both groups of clients. In particular, the gap in terms of accuracy is larger for the poor availability clients, especially at the early stages of the training. For both groups of clients, \texttt{FedFast} and \texttt{FedFNN} stabilize around the same level of accuracy, while \texttt{FedAvg} fails to reach the same level of accuracy for the poor availability group.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{plots/poor/legend.pdf}
    \begin{tabular}{cc}
    \hspace{-6mm}\includegraphics[width=0.55\linewidth]{plots/poor/normal.pdf} &
    \hspace{-6mm}\includegraphics[width=0.55\linewidth]{plots/poor/poor.pdf}\\
    (a) Always Available & (b) Poorly Available
    \end{tabular}
\caption{Simulation with poor availability clients subset , tested on FedFNN, FedFast and FedAvg. }
    \label{fig:pooravail}
\end{figure}


\paragraph{Sampling.} In this experiment we explore how different sampling rates affect the convergence of \texttt{FedFNN}, \texttt{FedFast} and \texttt{FedAvg}. Note that the sampling rate is the fraction of clients which participate in the training at each iteration. We choose 3 different sampling sizes, $\{1\%, 5\%, 20\% \}$. In Figure \ref{fig:sample} we present the experiments. For the smallest sample size (Fig. 5a) \texttt{FedFast} and \texttt{FedAvg} present high level of variability along all the training rounds, while \texttt{FedFNN} is stable, converging faster than \texttt{FedFast} and \texttt{FedAvg} to higher level of accuracy. For the other sample sizes (Fig. 5b and Fig. 5c) the differences in performance between \texttt{FedFNN} and the other algorithms still exists but it is increasingly diminished.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{plots/samplesize/legend.pdf}
    \begin{tabular}{ccc}
    \hspace{-3mm}\includegraphics[width=0.35\linewidth]{plots/samplesize/001.pdf} &
    \hspace{-3mm}\includegraphics[width=0.35\linewidth]{plots/samplesize/005.pdf} &
    \hspace{-3mm}\includegraphics[width=0.35\linewidth]{plots/samplesize/02.pdf}\\
    
    1\% Sample & 3\% Sample & 5\% Sample
    
    \end{tabular}
\caption{Simulations for Different Sampling Availability, tested on FedFNN, FedFast and FedAvg. }
    \label{fig:sample}
\end{figure}

\smallskip
\mybox{mygray}{ \begin{observation} \texttt{FedFNN} achieves better convergence for clients who have poor availability when compared to \texttt{FedFast} and \texttt{FedAvg}. It also converges much faster when adopting a small sampling rate (1\% or 5\%).
\end{observation}
}
\smallskip
 





==> source/intro.tex <==
\section{Introduction}
%Federated learning (FL) has recently attracted a lot of attention for training of machine learning models in a distributed fashion, when networks of remote devices communicates through a centralised server, which coordinates the information flow and update the machine learning model at each round (\newcite{fedfast},\newcite{kairouz2019advances}, \newcite{mcmahan2017communication}, \newcite{li2020federated}). 
%at each communication round, the server can interact only with a small portion of the whole pool of clients (e.g. when the mobile device is undercharge), and that sample changes at each iteration. Given the heterogeneity of data distribution among devices, most of the contributions in FL pose the attention on the importance of algorithm convergence, when data samples are not i.i.d. along the clients. 
%A constraint commonly posed on FL system is that client devices must be both charging and have an active Wi-Fi connection to participate in training. For this reason, only a small portion of the entire pool of clients can be sampled at each iteration, and this portion is dynamically changing during the learning process.
%Moreover, only a small portion of clients can be activated during each training round (\textbf{delegates}), while the vast majority of clients remain inactive (\textbf{subordinates}). In the case of recommendation algorithms' training, suggestions generated through a slow training process can lead to decrease in user engagement (e.g. because of delay in time to generate personalization), generating low user activity and thus less traffic for the new advertisement. This problem, faced during the training phase, less investigated but equally relevant, impacts the costs necessary, in terms of time and power, to implement the FL solution. 
%To address these challenges, a new line of work, \texttt{FedFast}, has been recently proposed.  
%\texttt{FedFast} uses ActvAgg for local model aggregation to replace the simple averaging, which speeds up the convergence by propagating the embedding updates from the selected clients to those unselected ones through a K-means clustering based method.
% represents the most relevant contribution, predicting the weights updates of the clients not directly involved in the training round, through a clustering based approach.
%In a separate line of research in meta-learning, a class of algorithms have been proposed to directly generate the weights of the target models \newcite{ha2016hypernetworks}.
%Inspired by these two lines of research works, we propose \texttt{FedFNN}, which introduces a meta network to learn to predict the embedding updates of the clients from local training. 
%This meta network can then be used to update the embeddings for the unselected clients in order to accelerate the FL.
%This will significantly slow down the learning of user and item representations. 
%As is shown in our experiments, the baseline FL method often needs many communication rounds before producing recommendations of reasonable quality. 
%
%In this scenario, \emph{data heterogeneity} and \emph{client availability} are two of the main challenges.
%
%The first is mainly due to distinct representations among users, which then lead to local training rounds generating biased representation, corrected only through the model aggregation happening on the server. 
%As a consequence of this effect, FL models need more iterations if compared to the centralized versions, to reach the same level of accuracy.
%The second is characterized by the small portion of clients that can participate in each training round, while the vast majority remains inactive. 
%Additionally, the training can happen only when the devices meet particular requirements (e.g. connected to an external power source, connected to Wi-Fi). 
%
%This phenomenon, also called \emph{poor client availability} slows down the training and reduce drastically the final performance of the model. Among many, \citeauthor{fedfast} \cite{fedfast} recently proposed a clustering based approach (\texttt{FedFast}) to reduce the amount of iterations to reach convergence in training.
%which relies on the assumption of having clustered embeddings in the input data distribution. Our solution is built upon a loose hypothesis, assuming similarity between clients embedding, not constrained by a clustered input data distribution.
%Our model improves in accuracy and speed of convergence the actual state-of-the-art (\texttt{FedFast}), which relies on the assumption of having clustered embeddings in the input data distribution. Our solution is built upon a loose hypothesis, assuming similarity between clients embedding, not constrained by clustered input data distribution. 
% \noindent\textbf{Contribution.} In this paper we propose \texttt{FedFNN}, a new framework for training recommender systems in FL settings. FedFNN is able to outperform the current state-of-the-art in both training speed and accuracy, using a supervised learning approach to predict unsampled client updates at each round of training. We extensively test the effectiveness of our solution on both synthetic and real data. 

\emph{Federated Learning} (FL) has become a pivotal formulation for distributing the computation of machine learning (ML) models in order to improve online services, such as content personalisation, and at the same time preserving user privacy.
%
This new paradigm is becoming extremely popular -- especially for use cases such as next word prediction or item suggestions -- since a personalised output can be generated on-device (e.g. smartphone, tablet, etc.), without the need to transfer sensitive data to an external server \cite{flanagan2020federated, mcmahan2017communication, ye2020edgefed, zhang2021subgraph}. 
%
In traditional, centralised learning approaches, private user data is transmitted to a central server and trained synchronously. In contrast, an FL setting involves computations being distributed among multiple devices through a server, which coordinates the training of the devices locally and aggregate their updates. This setting addresses privacy risks such as personal data leakage, misuse, or abuse, as client training data need not be disclosed to the central server. 
%
In an FL setting, mobile devices (\textbf{clients}) train their machine learning model locally, sharing only the model updates (and not the real historical data) with a centralised unique aggregator (\textbf{server}) \cite{fedfast, kairouz2019advances, mcmahan2017communication, li2020federated}.
%
The server then coordinates the training and distributes the model updates to clients at each round.
%
In this work, we specifically focus on the application of FL for recommender systems, which are trained on users' history data and make predictions on users' preference for candidate items. User and item data is usually represented through a low-dimensional embedding, which is a key component for most of the SOTA recommendation models \cite{ricci2011introduction, zhang2019deep}.
%
Figure 1a illustrates how FL models are trained. First (1a - Selected Client) a sample of clients are selected, where client history (1b - Client History) is converted in embeddings (2a - Embeddings) for the local training (2b - Local Training) and their embeddings are updated locally.
After the local training, the embedding updates are sent to the server (3a - Server), which aggregates the received updates (3b - Model Aggregated) and sends the new information to all clients to convert them in recommendations (4 - Recommendations).
%
\begin{figure}[t]
\begin{tabular}{cc}
    \hspace{-8mm}\includegraphics[width=0.45\linewidth]{imgs/fw1.png} &  \includegraphics[width=0.45\linewidth]{imgs/fw2.png}\\
    (a) FedAvg & (b) FedFNN
\end{tabular}
\caption{On the left, an illustration of the Federated Learning training process: $(1)$ the interactions of the client with the device are converted to vector embeddings (for both items and users); $(2)$ then the local training on the selected devices; $(3)$ the new training information are then sent to the server to be aggregated. $(4)$ the server sends the updates to all the clients which can generate the recommendations. On the right, the introduction of FedFNN, which generates the predictions of the unselected clients before sending the new updates.}
    \label{fig:idea}
    \vspace{-3mm}
\end{figure}

%\begin{figure}[t]

%    \centering
%    \hspace{-8mm}\includegraphics[width=1.1\linewidth]{imgs/framework.pdf}
%\caption{An illustration of the Federated Learning training process: $(1)$ the interactions of the client with the device are converted to vector embeddings (for both items and users); $(2)$ a portion of clients are selected and then run the local training on their devices; $(3)$ the new training information are then sent to the server to be aggregated. Specifically, $(3a)$ the server trains FedFNN prediction model on the local updates and (3b) aggregates the item embeddings; $(4)$ the server sends the $(4a)$ item embedding updates to the selected clients and $(4b)$ the new trained model to the unselected clients, which can locally generate client embedding updates' predictions. }
%    \label{fig:idea}
%    \vspace{-3mm}
%\end{figure}
%
This pipeline, proposed by \cite{mcmahan2017communication} represents the standard for training FL models in which, the representations for the trained users and items will be aggregated as an average on the server, before then being redistributed among untrained clients. 
%The asynchronous decentralized training represents the main bottleneck in FL, since it needs many communication rounds before producing recommendations of reasonable quality. 
%
Moreover, data characteristics in FL contribute to slow-down in training and decrease the model performance. In particular, we can distinguish: $(i)$ \emph{sparsity}, since most of the users interact only with a small portion of items; $(ii)$ \emph{heterogeneity}, since each client stores only the history of its own user; $(iii)$ low levels of client participation (\emph{poor client availability}), since at each training round only a small portion of clients can participate in the training (\textbf{delegates}), while the vast majority of clients remain inactive (\textbf{subordinates}). 
%
To cope with these issues, and as a result speed up the training, we propose \texttt{FedFNN}, a new algorithm that uses a meta network to learn and predict the embedding updates of the clients from local training. The proposed meta network can be used to update embeddings for unselected clients in order to accelerate the convergence (Figure 1b).
%
Our model consolidates preliminary recent results aiming at improving speed of the training \cite{fedfast}, proving to be superior in both speed of convergence and accuracy.
%
%In Figure 1b we show the differences between \texttt{FedFNN} and \texttt{FedAvg}. 
%\todo{change the figure and explain here the differences between FedAvg and FedFNN}

\texttt{FedFNN} model uses supervised learning approach to predict unseen clients updates at each round of the training, showing its effectiveness being tested on both synthetic and real data. We test our \texttt{FedFNN} algorithm on 3 different datasets, proving its effectiveness against the closest competitor (\texttt{FedFast}) and several baselines. We demonstrate that \texttt{FedFNN} is at least 5x faster (i.e. number of iterations to reach same level of accuracy). 
%
To test scenarios of low client availability and data sparsity, we introduce a synthetic data generator, which allows the artificial creation of user-item interaction data, comprised of distinct groups of clients which are defined by preference. We show how \texttt{FedFNN} is robust in terms of convergence speed and accuracy for different numbers of client groups and different levels of client availability.
%
We perform also an ablation study to shed the light on the contribution of several components introduced in \texttt{FedFNN}, in particular the ones regarding item updates aggregation and subordinates prediction. Our subordinates prediction method is the optimal choice, independent of the item update strategy.
%

\noindent\textbf{Paper Structure.} In the rest of this paper:  In Section ~\ref{sec:rw} we start by discussing the literature relevant to our work. In Section~\ref{sec:model} we introduce the background and formally define our proposed algorithm. In Section~\ref{sec:exp} we show the experimental setup and results. Finally, in Section~\ref{sec:disc} we conclude on our findings and discuss possible future directions. 
%we first discuss the literature relevant to our work in Section~\ref{sec:rw}. Then, we introduce the background and formally define our proposed algorithm in Section~\ref{sec:model}. The experimental setup and results are shown in Section~\ref{sec:exp}. Finally, we conclude this paper in Section~\ref{sec:disc}.

%\todo{emphasize that fedfast doesn't propose a method to predict efficiently the weights}



==> source/model.tex <==
\section{Preliminaries}
\label{sec:model}
%In this section we present our \texttt{FedFNN} algorithm, and describe also what differentiates it from \texttt{FedFast} and \texttt{FedAvg} algorithms.

Federated Learning is characterised by a unique server which handles incoming messages from multiple clients. The server aggregates these messages to optimise a single global optimum. In particular the objective is to minimise:
%
\begin{equation}
f(v,w) = \text{min } \sum_{k = 1}^N  p_k F_k(v, w)
\end{equation}
%
where $N$ is the number of devices, 
$v$ the item embeddings, 
$w$ the user embeddings,
$F_k(v,w)$ the local objective for the device $k$, which measures the local empirical risk over data distribution $D_k$,
and the normalisation factor $p_k \in [0,1]$ applied to $F_k(v,w)$. 
%
The learnable parameters are $\{v, w, \phi \}$, where $\phi$ is the set of all the other less relevant parameters, needed to train the General Matrix Factorisation (\texttt{GMF}) algorithm. 
%
This model is widely used in designing recommendation algorithms and predicts user preferences through a low-dimension representation of the data. 
%
To learn the user preferences from the embeddings, it uses a fully connected layer that takes as input user and item embeddings and outputs the scores distribution for all the missing interactions \cite{he2017neural}.
%To learn the user preferences from the embeddings, a fully connected layer is used, which takes as input user and item embeddings, and outputs the scores distribution for all the missing interactions \cite{he2017neural}.

%This model can then be naturally extended in a federated setting, using \texttt{FedAvg}, where a subset $S$  of all devices N are selected for the local updates. In Algorithm \ref{algo:flalgo} we present the steps included in a Federated Learning approach based on \texttt{FedAvg}. 
This model can then be naturally extended in a federated setting using \texttt{FedAvg}, where a subset of all devices are selected for local updates. 
Algorithm \ref{algo:flalgo} presents the steps of \texttt{FedAvg};
%At each iteration, first a bunch of clients are sampled (line 3), and then locally updated (line 4). Those clients are then used for predicting the unsampled ones (lines 7-8) and the remaining item updates are aggregated and updated (lines 9-10). More precisely, in \texttt{FedAvg} the item updates are generated through a weighted average of all the clients, and unsampled clients are not updated; while in \texttt{FedFast} and \texttt{FedFNN} introduce distinct strategies for predicting those clients.
%The sampled clients are also called  \textbf{delegates}, while the remaining ones are the \textbf{subordinates}. 
%When a client is not sampled for a single round in \texttt{FedAvg}, it does not update the training weights on the device for that round.
each $k$-th sampled client (line 3) gets first a copy of the model to train on its own local data $D_k$, and subsequently the loss function $L$ optimised by the local model with respect to $\{v_k, w_k, \phi_k \}$ (lines 4,5):
%
\begin{equation}
\{v_k, w_k, \phi_k \} \leftarrow  \textbf{ A }(v, w, \phi, L, D_k),  \text{  for each } k \in S, 
\end{equation}
%
where $(v_k, w_k, \phi_k)$ are the learnable parameters updated by the delegate client $k$, \textbf{A} is the optimisation algorithm selected to estimate the parameters values and 
$S \subseteq \{1, \ldots, N\}$ is the indices of all the delegates. 
%
Since we work with implicit feedback data, a binary cross-entropy loss function is selected; for the optimisation algorithm the ADAM optimiser is chosen.

For each training round, the weights updated through the local models are aggregated to generate the global update (lines 6-10). In particular, among all the client embeddings included in the global model $w[D]$, when using \texttt{FedAvg}, only the embeddings of the delegates  $S$ (i.e. $w_k[k], k \in S$) will be updated: 
%
\begin{equation}
w^\textit{new}_k[k] \leftarrow w_k[k], \text{ for each } k \in S 
\end{equation}
%
In contrast, the item embeddings are aggregated in the server (lines 9-10) and then redistributed among all the clients.

\begin{algorithm}[t]
  \caption{\textsc{FL Algorithm} }
  \label{algo:flalgo}
  \Input{set of item $I$, set of clients $U$, sample size $m$}
  %interactions $D$, 
  %\Output{A set $O$ of $k$ rewiring operations}
  Initialise: user embeddings $w_1$, item embeddings $v_1$\;
  \For{$t \gets 1,2,\ldots,T$}{
    $S_t \gets$ ClientSampling($U$, $m$)\;
	\For{client $k \in S_t$}{
	  $w_k^{t+1}, v_k^{t+1}  n_k \gets$ LocalUpdate($w^t_k,v^t_k, k$)\;
    }
    $\Omega_t \gets w^{t+1}, S_t, m$\;
    \For{client $j \in U \backslash S_t$}{
	  $w_j^{t+1}, n_k \gets$ ClientPrediction($\Omega_t$)\;
    }
    %\For{item $i \in I$}{
	%  $v_i^{t+1} \gets$ %ItemUpdate($v^t_i$, %$v^t[S_t]$)\;
	$v^{t+1} \gets$ ItemUpdate$( v^t[S_t])$\;
    %}
  }
\end{algorithm}

Updating only a subset of clients represents a limitation that affects the number of rounds necessary to get good model performances. In this direction, subordinate clients updates are crucial to the convergence of the global model. 
In \texttt{FedAvg} the embeddings of the local clients are updated as follows:
%
\begin{equation}
w^{\textit{new}}[j] \leftarrow \frac{1}{|S|} \sum_{k \in S} w_k[k],  \text{  for each } j \in U \setminus S
\end{equation}

%In order to predict the unsampled clients embeddings, a clustering-based approach (\texttt{FedFast}) has been recently proposed, which aims at inferring the updates of the subordinate users averaging the weight update between users belonging to the same cluster of preferences. 
%In order to make update to the unselected clients embeddings, a clustering-based model aggregation approach (\texttt{FedFast}) has been recently proposed, which updates the embeddings of subordinate users with the averaged weight update of the selected users belonging to the same cluster.
To update embeddings of subordinate clients, \texttt{FedFast} recently proposes a clustering-based model aggregation approach to update the embeddings of subordinate users with the averaged weight update of the selected users belonging to the same cluster \cite{fedfast}.
%The assumption is that if two users are close in the embedding space, their embeddings will have similar updates after local learning. If we consider the task of predicting the subordinates as a regression problem, using the local updates from user embeddings, the FedFast solution is essentially solving the regression problem by clustering. 
First, users are clustered based on their embeddings $C = \{c_i \mid i = 1, 2, \ldots\}$, 
where each cluster $c_i$ is a set of users. 
Then, the averaged weight update $\delta_{c_i}$ is computed for all clients in $c_i$:
%
\begin{equation}
\delta_{c_i} \leftarrow \frac{1}{|c_i \cap S|}\sum_{k \in c_i \cap S} w_k[k] - w[k], \text{ where  } i = 1, 2, \ldots, |C| 
\end{equation}

The new averaged update is used for modifying the weights of the subordinate users:  
%
\begin{equation}
w^{\textit{new}}[k] \leftarrow w[k] + \delta_{c_i}, \text{ for each } k \in c_i \setminus S 
\end{equation}

%The detalied process is presented in Algorithm\ref{algo:fedfast}.

Despite being faster to converge than \texttt{FedAvg}, \texttt{FedFast} relies on two assumptions which may be difficult to maintain consistently: 
\emph{(i)} it assumes that clients can be clustered into distinct groups, which is not always the case (e.g. group of users presenting highly overlapping preferences); 
\emph{(ii)} even upon assuming the existence of the groups of preferences, fixing an \emph{a priori} number of clusters for the sampled clients relies on the feasibility to sample users from all the clusters at each round.
%\emph{(ii)} even upon assuming the existence of the groups of preferences, fixing an \emph{a priori} number of clusters for the sampled clients relies on the idea that at each round it is possible to sample users from all the clusters. 

Moreover, since real data cannot be accessed in a unique pass, finding the correct number of clusters in the federated setting may require multiple tests before the final model training. 
Due to these limitations, as is found in our ablation study in Section~\ref{sec:exp}, 
their cluster-based update propagation produces little to no improvements over the training of the models.



%%%%%%%%%%%%%%%%%%%
%%% NEW SECTION %%%
%%%%%%%%%%%%%%%%%%%

\section{FedFNN}
%To overcome those limitations, we propose \texttt{FedFNN}, a model which assumes no dependency from the clustered preferences.
To overcome the limitations mentioned above, we relax the assumption of the clustered preferences to the assumption that if two users are close in the embedding space, their embeddings would have similar updates after local learning. 
Under this new, relaxed assumption, we propose \texttt{FedFNN} that directly predicts the embedding weight updates for subordinates using supervised regression models. 
This idea is also closely related to the class of meta-learning algorithms which directly generates the weights of the target model \cite{ha2016hypernetworks, zhang2018graph}.
However, instead of directly generating the embedding weights,
\texttt{FedFNN} predicts the embedding updates using those produced by the delegate clients. 

The training phase is performed on the data coming from the delegates to optimise a learning function $f(\cdot; \theta)$, using the previous user embeddings as input variable and the new embeddings updates as output:
%
\begin{equation} \label{eq:main}
\arg \min_{\theta} \mathbb{E}_{U} \ell\big(f(w[U]; \theta), w^{\textit{new}}[U] - w[U]\big)
\end{equation}
%
The objective function is the expected RMSE taken over the distribution of all the clients $U$ as we are interested in the generalisation error of the update predictor. The architecture for $f(\cdot; \theta)$ proposed in the experiments with FedFNN is a multi-layer perceptron (MLP), which proves to be simple but effective with the datasets we use. %, however, in the Appendix we also test different configurations including RNN and CNN.


%$$
%\theta^* \leftarrow \arg \min_{\theta} \sum_{k \in S} \ell(g(w[k]; \theta), w^{new}[k] - w[k])
%$$

Then, for each subordinate client we predict the updates
%
\begin{equation}
w^{\textit{new}}[j] \leftarrow e^{- \gamma t }  \ell(w[j]; \theta^*)  + (1 - e^{- \gamma t }) w[j] , \text{ for each } j \in U \setminus S
\end{equation}
%
where $\gamma$ is the discount factor and $t$ the number of running epochs. 
Both of these parameters are combined to generate an exponential decay and reduces the contribution of the new predictions after each iteration. 
The updates are predicted by minimising the error produced on average (RMSE) and since weights need to converge towards personalised values dependent on the client information, 
those predictions becoming less relevant in the long-run.

In contrast to \texttt{FedFast}, which uses unsupervised learning (e.g., k-means), \texttt{FedFNN} uses supervised learning that explicitly models the mapping from the client representation to the user embedding updates.
%
Additionally, \texttt{FedFNN} enables the introduction of more sophisticated machine learning models (e.g. Neural Networks), adding the ability to capture more information and increasing modeling power. 
% Later, we show through an ablation study that the unsupervised learning does not generate such a dramatic improvement over the training of the models.
Later, we show through an ablation study that updating the subordinate client embedding using \texttt{FedFNN} can generate significant improvements over the training of the models, which is not the case for the clustering method.

\subsection{Optimisation} 

%\noindent \textbf{Optimization.} 
% Since in a FL setting, the local training is performed without accessing the entire dataset, the architecture parameters of \texttt{FedFNN} can not be fixed before the starting of the global training. For this reason, we propose that during each round of prediction for \texttt{FedFNN}, we include hyperparameter optimization for. In this way input parameters can be optimized accordingly with the updates generated through the local training. We use grid-search with 5-fold cross validation, optimizing the learning rate, the dropout, and the number of hidden neurons. 
%The evaluation and optimization of Eq.~\ref{eq:main} requires taking the expectation over the distribution of all the clients, which is not practical in practice.
To find the optimal parameter $\theta$ in Eq.~\ref{eq:main}, we adopt a standard supervised learning approach based on cross validation. More specifically, for each communication round, we run 5-fold cross validation on the delegate clients, train $f(\cdot;\theta)$ on the training set using SGD based optimisation methods and approximate the objective in Eq.~\ref{eq:main} with the empirical loss on the validation set. During each round, we use grid-search to optimise the hyper-parameters on the validation set. Our set of hyper-parameters include: the network architectures, learning rates and dropout ratios for regularisation.
Moreover, since FedFNN is designed to optimise the training of the global model at early stage of the iterations, we use a \emph{patience} parameter $p$, similar to the early-stopping criteria used to avoid overfitting in supervised learning (\newcite{prechelt1998early}), to stop predicting the subordinates embeddings. Specifically, at each iteration $t$ we monitor the loss function value of the global model with respect to the value at iteration $(t-p)$. Once the loss function stabilizes around a previous value, we stop using FedFNN. More precisely, we stop using FedFNN when $|1 - L(t)/L(t-p)| < \epsilon$ (where $\epsilon  = 0.01$), where $L$ represents the loss function of the global model. Algorithm \ref{algo:fedfnn} presents the whole process.

%\todo{redo a pass here - explaining the choice of the algorithm, CV, etc...}

For the item updates, various  strategies can be applied to define the importance of the local update generated through the client $k$. Specifically, a coefficient $\alpha_k$ can be defined for each delegate client. In particular we implement \texttt{FedFNN} along with 3 different strategies:

\begin{itemize}
\item\textbf{W0}: The new local embedding updates are re-distributed through averaging the new changes among all the sampled items, where $\alpha_k = 1/m$, $\forall k \in S$

\item\textbf{W1}: The local item updates are distributed following the weighted average proposed in \cite{fedfast}, where the importance of weights updates in the current iteration is distributed according to the difference between the update and the embedding. 
Let 
%
\begin{equation}
Z_{t+1}[k] = \sum_{v_i \in D_k} ||v^i_{t+1}[k] - v^i_{t}||_1.
\end{equation}
%
Then, we set
\begin{equation}
\alpha_k = \frac{Z_{t+1}[k]}{\sum_{k \in S_t} Z_{t+1}[k]}.
\end{equation}
%
In this way, the clients presenting bigger updates are valued more.


% In this case $\alpha_k = U_{t+1}[k] /\sum_{k \in S_t} U_{t+1}[k]$, where
% %
% \begin{equation}
% U_{t+1}[k] = \sum_{v_i \in D_k} ||v^i_{t+1}[k] - v^i_{t}||_1
% \end{equation}
% %
% In this way the clients presenting bigger updates are valued more.

\item\textbf{W2}: The local item updates are weighted by the number of samples included in each delegate client, where $\alpha_k = \frac{n_k}{\sum_k n_k}$, where $n_k$ is the number of interactions present in the client history.
%\item\textbf{W3}: The method proposed here is a combination of W1 and W2. The average is weighted by both the relative number of interactions and the size of the item update.


\end{itemize}

\subsection{Sampling} 
%\noindent\textbf{Sampling. } 
In contrast to the \texttt{FedFast} algorithm, we do not add any constraint to the sampling strategy. We assume that in a practical, real use case scenario, sampling would be determined via external factors (e.g. client availability, connection quality, etc), not the algorithm being used. 

\begin{algorithm}[t]
  \caption{\textsc{FedFNN} }
  \label{algo:fedfnn}
  \Input{$\Omega_t \leftarrow\{ W_{t}, S, W_{t+1}[S]\}$, prediction function $g(.)$, number of delegates $m$, patience criteria $p$}
  \Output{$W_{t+1}[D]$, $RMSE_t$}
  \If{$t \leq p$ \textbf{or} $|1 - L(t)/L(t-p)| \geq \epsilon$}{
    $\delta[S] \leftarrow W_{t+1}[S] - W_t[S]$\;
    $\theta^*, RMSE_t \leftarrow \arg \text{ opt}_{\theta} \sum_{k \in S} \ell(g(w_t[k]; \theta), \delta[k])$\;
    \For{client $j \in D \backslash S_t$}{
      $w_{t+1}[j] \leftarrow e^{- \gamma t }  g(w_t[j]; \theta^*)  + (1 - e^{- \gamma t }) w_t[j]$\;
    }
  }
%\caption{FedFNN Client Prediction}
\end{algorithm}


















==> source/rw.tex <==
\section{Related Work}
\label{sec:rw}

\subsection{Federated Learning}

Federated Learning has emerged recently as popular research area, since it allows exploitation of the vast amount of data collected on personal devices through privacy-preserving technologies \cite{kairouz2019advances, li2020federated}. 
%
\citeauthor{mcmahan2017communication} was the first to introduce the definition of Federated Learning, 
with the Federated Averaging (\texttt{FedAvg}) algorithm that is capable of increasing the training speed of classification models through the sharing of weight updates among sampled clients \cite{mcmahan2017communication}. 
%
The \texttt{FedAvg} algorithm has been applied to various fields, such as natural language processing (NLP), Computer Vision (CV) and recommender systems. 
For this reason, many contributions have been proposed recently, aimed at modifying and improving \texttt{FedAvg} \cite{li2019convergence, qu2020federated, zhong2021p, karimireddy2020scaffold}.

Parallel to the \texttt{FedAvg} improvements, there is a new line of work proposing increased accuracy of models in the presence of heterogeneous data distributions among devices (i.e. an imbalanced distribution of samples among the different devices), also called \emph{statistical heterogeneity} \cite{li2018federated, wang2020tackling, karimireddy2020scaffold}. \citeauthor{li2018federated} propose \texttt{FedProx}, which modifies \texttt{FedAvg} algorithm by including a proximal term, reducing differences between local and global updates \cite{li2018federated}. 
\citeauthor{wang2020tackling} propose \texttt{FedNova}, a method that eliminates objective inconsistency through normalised averaging \cite{wang2020tackling}. 
The definition of statistical heterogeneity introduced by them is not directly translatable to the recommendation systems settings, making the aforementioned methods not comparable to \texttt{FedFNN}. 

% continue from here

A parallel line of work focuses on improving on-device personalisation of FL models \cite{li2021ditto, pmlr-v97-mohri19a, jiang2019improving, deng2020adaptive}. 
It is worth noting that personalisation lies close to fairness; the latter aims at reducing the variability of performance across clients \cite{li2021ditto}. 
As \texttt{FedFNN} focuses on improving the training speed, we believe that our work is complementary.
% which aims at reducing variance in performance across clients \newcite{li2021ditto}. As for the previous line of research, \texttt{FedFNN} can not be directly compared with those methods, since we pose the focus on the speed of training phase.

\subsection{Federated Learning in Recommender Systems}

The FL paradigm has been mainly investigated for supervised learning tasks (e.g. binary and multi-label classification). Due to its effectiveness of generating on-device personalised recommendations without violating the user privacy, it has also been applied to the area of information retrieval and recommendation algorithms \cite{wu2021fedgnn, fedfast, anelli2021federank, kalloori2021horizontal, liang2021fedrec++}.

Most of the contributions focus on the matrix factorisation algorithm, which represents the standard to capture latent dimensions of user-item interactions \cite{he2017neural, koren2009matrix}.
%
\citeauthor{anelli2021federank} introduce \texttt{FedeRank}, a federated recommendation algorithm  which allows users to control the portion of data they want to share \cite{anelli2021federank}; 
it focuses on the accessibility of personal data, which is an aspect not covered by \texttt{FedFNN}. 
%
\citeauthor{lin2020fedrec} propose \texttt{FedRec}, a federated model for predicting explicit feedback \cite{lin2020fedrec}; in contrast, our work focuses on implicit feedback. 
Additionally, their objective is to generate performances as close as possible to the centralised version of the model, whereas our focus is to improve training speed. 
%
%\citeauthor{ammad2019federated} proposed a federated version of the multi-view matrix factorization algorithm, to improve the level of personalization. \texttt{FedFNN} is not designed for multi-view data, so it is not directly compared.

%The work probably most relatable to ours is the \texttt{FedFast} algorithm, proposed by \cite{fedfast}. 
\citeauthor{fedfast} propose \texttt{FedFast} algorithm that proposes to
to speed up the recommender system training by clustering the users \cite{fedfast}. 
Specifically, they propose: 
$(i)$ a model to update unsampled clients, 
$(ii)$ an item update strategy which looks at client contribution weighting and 
$(iii)$ a sampling technique that is coherent with the clustering approach. 
%
Compared to our work, they rely on the assumption of having clustered embeddings in both, the input data distribution and the clients sampled for the local update. We show through an ablation study how their clustering approach does not significantly help in the prediction task, presenting performances close to the baseline (with no prediction for the unsampled clients).
%
Our work aims to capture similarities at individual and not group level, between user embeddings. 
We extensively compare \texttt{FedFNN} to \texttt{FedFast} in Section~\ref{sec:exp}, 
showing the effectiveness of our solution. 

\texttt{FedFNN} intuition is built on the idea of predicting differences in the next weights updates of the subordinate clients, which intuitively can be connected to \cite{He_2016_CVPR}, a popular architecture achieving state-of-the-art performances in Computer Vision tasks, where the hidden layers are enhanced with the prediction of the difference between the new and old weights. \citeauthor{ha2016hypernetworks} proposes hypernetworks, strongly related to our work, where a single network is used to generate the weights of another architecture \cite{ha2016hypernetworks, zhang2018graph}. 
%
In hypernetworks, one architecture is trained and the other predicted, while in our case, \texttt{FedFNN} is trained to predict the updates of the weights of the main model, which then uses the updates for the local training. 
%
Another relevant line of research connected to hypernetworks is meta-learning, which has been also explored in connection with Federated Learning~\cite{lin2020meta,chen2018federated}. 
Specifically, in those approaches a meta recommender system is designed, able to generate item embeddings with a meta network.

\texttt{FedFNN} is built on Matrix Factorisation algorithm, which represents the standard for recommender systems in presence of implicit feedback \cite{koren2009matrix}. However recently, models more sophisticated than that have also been proposed. Among many, \citeauthor{wu2020fedctr} introduced a federated framework for online advertising to 
predict CTRs of native ads from multi-platform user behavior \cite{wu2020fedctr}, 
while \citeauthor{wu2021fedgnn} introduce a graph neural network architecture to predict high-order user interactions \cite{wu2021fedgnn}. \texttt{FedFNN} can be extended to other sophisticated models in a FL setting and we leave this task for the future work.

%Algo 3 similar to FedFast \cite{ji2019learning} 
%amazon-data \cite{mcauley2015image}

